Form factors at strong coupling via a Y-system

We compute form factors in planar N=4 Super Yang-Mills at strong coupling. Namely we consider the overlap between an operator insertion and 2n gluons. Through the gauge/string duality these are given by minimal surfaces in AdS space. The surfaces end on an infinite periodic sequence of null segments at the boundary of AdS. We consider surfaces that can be embedded in AdS_3. We derive set of functional equations for the cross ratios as functions of the spectral parameter. These equations are of the form of a Y-system. The integral form of the Y-system has Thermodynamics Bethe Ansatz form. The area is given by the free energy of the TBA system or critical value of Yang-Yang functional. We consider a restricted set of operators which have small conformal dimension.

==> toc.tex <==
\noindent {1.} {Introduction} \leaderfill{2} \par
\noindent {2.} {Short review of the strong coupling prescription for computing form factors} \leaderfill{5} \par
\noindent {3.} {Derivation of the Y-system for general monodromy} \leaderfill{6} \par
\noindent \quad{3.1.} {Preliminaries} \leaderfill{6} \par
\noindent \quad{3.2.} {Kinematics of the general problem} \leaderfill{11} \par
\noindent \quad{3.3.} {Truncation of the Y-system} \leaderfill{12} \par
\noindent \quad{3.4.} {Normalization independent definition of the Y-functions} \leaderfill{13} \par
\noindent {4.} { Constant monodromies} \leaderfill{15} \par
\noindent \quad{4.1.} {Recovering the Y-system for scattering amplitudes} \leaderfill{16} \par
\noindent \quad{4.2.} {Y-system for the form factors of operators with small dimension} \leaderfill{16} \par
\noindent \quad{4.3.} {Y-system for ${\rm Z}_{m}$ symmetric solutions} \leaderfill{17} \par
\noindent {5.} { Y-system for the form factors} \leaderfill{18} \par
\noindent \quad{5.1.} {Zig-zag solution} \leaderfill{18} \par
\noindent \quad{5.2.} {Analytic properties of the Y-functions} \leaderfill{21} \par
\noindent \quad{5.3.} {Evaluating Y's} \leaderfill{22} \par
\noindent \quad{5.4.} {Integral form of the equations} \leaderfill{24} \par
\noindent {6.} {Area in the case of form factors} \leaderfill{25} \par
\noindent \quad{6.1.} {General formula} \leaderfill{25} \par
\noindent \quad{6.2.} {Area as the free energy} \leaderfill{26} \par
\noindent \quad{6.3.} {Area as the critical value of Yang-Yang functional} \leaderfill{26} \par
\noindent {7.} {Exact solutions} \leaderfill{27} \par
\noindent \quad{7.1.} {High temperature limit of the form factor Y-system} \leaderfill{28} \par
\noindent \quad{7.2.} {High temperature limit of the ${\rm Z}_{m}$ symmetric Y-system} \leaderfill{29} \par
\noindent \quad{7.3.} {Exact solution for the $4$-cusp form factor} \leaderfill{30} \par
\noindent {8.} {Conclusions} \leaderfill{33} \par
\noindent {9.} {Acknowledgments} \leaderfill{34} \par
\noindent Appendix {A.} {Derivation of the monodromy} \leaderfill{34} \par
\noindent Appendix {B.} {${\rm Z}_{m}$} symmetric polygons \leaderfill{36} \par
\noindent Appendix {C.} {Computation of $A_{cut-off}$ for $n$ odd} \leaderfill{37} \par
\noindent Appendix {D.} {Integral equations for complex masses} \leaderfill{39} \par
\noindent Appendix {E.} {Calculation of $N=4k$ gluon amplitudes by taking the double soft limit} \leaderfill{39} \par
\noindent \quad{\hbox {E.}1.} {Soft limit of the $A_{0}$} \leaderfill{42} \par
\noindent \quad{\hbox {E.}2.} {Soft limit of the $A_{BDS-like} - A_{BDS}$} \leaderfill{42} \par
\noindent \quad{\hbox {E.}3.} {The octagon} \leaderfill{45} \par
\noindent Appendix {F.} {On the connection with BTZ black holes} \leaderfill{46} \par
\noindent Appendix {G.} {The monodromy in terms of coordinates} \leaderfill{47} \par


